Privacy-Preserving Individual-Level COVID-19 Infection Prediction via Federated Graph Learning

Accurately predicting individual-level infection state is of great value since its essential role in reducing the damage of the epidemic. However, there exists an inescapable risk of privacy leakage in the fine-grained user mobility trajectories required by individual-level infection prediction. In this paper, we focus on developing a framework of privacy-preserving individual-level infection prediction based on federated learning (FL) and graph neural networks (GNN). We propose Falcon, a Federated grAph Learning method for privacy-preserving individual-level infeCtion predictiON. It utilizes a novel hypergraph structure with spatio-temporal hyperedges to describe the complex interactions between individuals and locations in the contagion process. By organically combining the FL framework with hypergraph neural networks, the information propagation process of the graph machine learning is able to be divided into two stages distributed on the server and the clients, respectively, so as to effectively protect user privacy while transmitting high-level information. Furthermore, it elaborately designs a differential privacy perturbation mechanism as well as a plausible pseudo location generation approach to preserve user privacy in the graph structure. Besides, it introduces a cooperative coupling mechanism between the individual-level prediction model and an additional region-level model to mitigate the detrimental impacts caused by the injected obfuscation mechanisms. Extensive experimental results show that our methodology outperforms state-of-the-art algorithms and is able to protect user privacy against actual privacy attacks. Our code and datasets are available at the link: https://github.com/wjfu99/FL-epidemic.

==> 6.discussion.tex <==
\section{Discussion}\label{sec::discussion}

\subsection{Implications and Applications}
% Epidemic simulation traditionally serves as one of
% the important methods to forecast how an epidemic may spread
% among a population. However, there are two key limitations that
% restrict the scope of such methods. The first limitation is that
% the existing tools rely on different sets of static parameters (e.g.,
% infection probability, recovering probability) for simulating an
% epidemic spread that may fail to capture the dynamic nature
% of population interactions that acts as a dominant factor in an
% epidemic spread scenario such as COVID-19 pandemic. To handle
% this challenge, we propose a machine learning based model that
% combines a Graph Convolutional Neural Network (GCN) and
% a Recurrent Neural Network (RNN). It integrates the ability of
% the GCN to capture spatial dependency in human interaction
% and the ability of the RNN to incorporate temporal effects of
% the virus spread. The second limitation is that these methods do
% not address the computation overhead problem when dealing
% with time-dynamic graphs. Training a GCN on a very large
% graph suffers from the communication overhead from different
% graph partitions and the computation overheads stemming
% from partitioning dynamic graphs. This limitation impacts the
% scalability of the existing systems. To solve this challenge, we
% partition the graph in a computationally less expensive manner by
% partitioning the graph using the min-cut principle. We conducted
% comprehensive large scale real-world human mobility data driven
% experiments. Our experimental result shows that the proposed
% machine learning based forecasting model achieves overall 84%
% classification accuracy with greater than 72% precision and 62%
% recall. Also, the proposed graph partitioning approach reduces
% computation time and commutation overhead by a significant
% margin.
In this paper, we proposed an individual infected detection method to exploit individual infectious risks from mobility data. It is worth mentioning that our work has contributed a lot to understanding the interaction between mobility patterns and epidemic spread, which validates the feasibility of using mobility data for epidemic forecasting. And our research result has the strong characteristic of practicality and applicability in the real world. This work can be used in isolation policies~\cite{bahr2009exploiting}, distribution of influenza vaccine to high-risk groups~\cite{ompad2006distribution}, feedback strategies~\cite{di2020covid} and avoidance of the generation of clusters~\cite{shim2020transmission}. Moreover, We protect user privacy while using mobile trajectory data to predict the infectious risk of individuals, which is strongly demanded in pandemic research~\cite{yin2017location, veliz2021privacy}. Thus, it further improves the feasibility of real anti-epidemic work. And we also analyze the inner relationship between the infected ratio and user mobile behavior patterns. It also gives significant advice for epidemic prevention and control.
% In the stage of technology, we propose a new way of constructing epidemic hypergraph and a novel causal aware propagation mechanism based on HGNN. It solves the problem that traditional graph neural networks such as GCN cannot handle the complex relationship between users and regions and cannot process the complex temporal features in the real epidemic spread. Additionally, we introduce differential privacy mechanism to protect user privacy, and a confidence-aware mechanism is proposed to restrict the performance loss produce by Obfuscated mechanism. We outperform existing algorithms on multiple classification algorithm metrics and one metric we designed for the epidemic spread task. Then we analyzed the impact of the embedding size and time interval hyperparameters on our performance through experiments and provided the recommended hyperparameter design. We also grouped users in various ways and analyzed the different predictive performances of our model for different types of users.
\subsection{Limitations}
Despite the novelty of our research, there are also some limitations to this work.
In this study, we principally obtain our research findings from one mobility dataset collected by WeChat from the city of Beijing. And we observed three biases in this dataset, including temporal domain, spatial domain, and individual domain. In the temporal domain, the mobility dataset was collected in 2016, and the mobile patterns of the population may have changed. In the spatial domain, there might be bias due to the city’s traditional lifestyle and cultural background. And these mobile trajectories are gathered by using apps on mobile phones, and human trend to frequently use social media services in some places, like office buildings and commercial districts. Thus, the data we obtain will be dense in this area. In the individual domain, the dataset was collected by a private enterprise. Thus, it only includes the mobility data of users who use the app developed by Tencent. This subpopulation may not reflect the population comprehensively.
Summarizing the arguments, inevitable noise and biases may be brought in our experiments. In fact, we utilize several approaches to reduce the influence of the limitation and provide more credible results. As for the bias brought by the data location distribution, we have chosen an area and deleted some users with sparse trajectories. 
A causal mechanism is proposed to only address the spatial dependency of epidemic spread, but we do not consider the causal effect in the output layer. 
Although our infected detection result validates the effectiveness of our model, the features we used only include user mobility data when other characteristics like age, gender, and physical condition are not taken into consideration. Moreover, our model benefit from the casual mechanism, the output features of a user are chronological, but we do not use this character to further improve our model.

% 收集数据的时间2016
% 只有部分人的打卡数据
% 打卡数据稀疏 
% 打卡时间上的bias
% 没有考虑用户的其它体征,年龄，性别，身体状况，

\subsection{Future Works}
In order to address the above limitations, there is some improvement we plan to accomplish in the future. First, there is some bias in our mobility data, and we plan to collect wireless base data access data from ISP, which has more comprehensive users and lower spatial bias. Second, the potential of our proposed causal mechanism has not yet been completely exploited. We will try to use intermediate infectious data to improve the performance of our model further. Third, we have the layout to take the other features, like age, gender, and physical condition into consideration. Note that these data are also private information, and we plan to use anonymous models~\cite{sweeney2002k,xiao2007m,li2007t,machanavajjhala2007diversity} to provide sufficient privacy.
